New Codes on High Dimensional Expanders

We describe a new parameterized family of symmetric error-correcting codes with low-density parity-check matrices (LDPC). Our codes can be described in two seemingly different ways. First, in relation to Reed-Muller codes: our codes are functions on a subset of $\mathbb{F}^n$ whose restrictions to a prescribed set of affine lines has low degree. Alternatively, they are Tanner codes on high dimensional expanders, where the coordinates of the codeword correspond to triangles of a $2$-dimensional expander, such that around every edge the local view forms a Reed-Solomon codeword. For some range of parameters our codes are provably locally testable, and their dimension is some fixed power of the block length. For another range of parameters our codes have distance and dimension that are both linear in the block length, but we do not know if they are locally testable. The codes also have the multiplication property: the coordinate-wise product of two codewords is a codeword in a related code. The definition of the codes relies on the construction of a specific family of simplicial complexes which is a slight variant on the coset complexes of Kaufman and Oppenheim. We show a novel way to embed the triangles of these complexes into $\mathbb{F}^n$, with the property that links of edges embed as affine lines in $\mathbb{F}^n$. We rely on this embedding to lower bound the rate of these codes in a way that avoids constraint-counting and thereby achieves non-trivial rate even when the local codes themselves have arbitrarily small rate, and in particular below $1/2$.

==> unused/code_rate_old.tex <==
\subsection{Rate of Local Code at a Vertex}
%
%
In this section we analyse the rate and local testability of the code $C_{q,d_x,d_y}\subseteq \set{ f:\F_q^3\to\F_q}$ defined in \eqref{eq:def:vertexcode}.



Since $f(x, b, c)$ lies on a degree $d$ polynomial in $x$ for any $b, c$, we can write $f(x, y, z)$ as a polynomial that is degree $d$ in $x$ and degree $p-1$ in $y$ and $z$:
\[
    f(x, y, z) = \sum_{\substack{0 \le i \le d \\ 0 \le j, k \le p-1}} c_{ijk} x^i y^j z^k.
\]
Plugging in $(x, y, xy + z)$, we get that 
\[
    f(x, y, xy + z) = \sum_{\substack{0 \le i \le d \\ 0 \le j, k \le p-1}} c_{ijk} x^i y^j (xy + z)^k.
\]
We can reduce $f(x, y, xy + z)$ modulo $y^p - y$ to get a polynomial $g(x, y, z)$ that is degree $\le p-1$ in $y$ and $z$, and $\le d+p-1$ in $x$. Write
\[
    g(x, y, z) = \sum_{0 \le j \le p-1} g_j(x, z) y^j
\]
where $g_j(x, z)$ is degree $p-1$ in $z$. The condition that $f(a, y, ay+c)$ lies on a degree $d$ polynomial in $y$ for all $a$ and $c$ means that $g_j(x, z) = 0$, where $d < j \le p-1$, for all $x, z$. In particular, if we write $g_j(x,z) = \sum_{0 \le k \le p-1} g_{jk}(x)$, where $g_{jk(x)}$ a degree $\le p-1+d$ polynomial that is the coefficient of $y^jz^k$ in $g(x,y,z)$, then if we know that $g_{jk}(x)$ is degree $\le p-1$ in $x$, then in fact all coefficients in $g_{jk}(x)$ must be $0$. We will use this fact extensively in the analysis of the rate.

First, we will need the following lemma.

\begin{lemma} \label{lemma:invertible_matrix}
    Assuming that $r \le k \le m < p$, the following matrix has full rank:
    \[
        \begin{pmatrix}
            \binom{m}{k} & \binom{m}{k-1} & \cdots & \binom{m}{k-r} \\
            \binom{m-1}{k} & \binom{m-1}{k-1} & \cdots & \binom{m-1}{k-r} \\
            \vdots & \vdots &  & \vdots \\
            \binom{m-r}{k} & \binom{m-r}{k-1} & \cdots & \binom{m-r}{k-r}
        \end{pmatrix}
    \]
\end{lemma}

\begin{proof}
    We divide the entries of row $i$ by $(m-i)!$ (where the top row is row $0$), and multiply the entries of column $j$ by $(m-k+j)!(k-j)!$ (where the leftmost column is column $0$). Since $m < p$, both $(m-i)!$ and $(m-k+j)!(k-j)!$ are nonzero. We obtain that the rank of the above matrix is equivalent to the rank of the below matrix:
    \[
        \begin{pmatrix}
            1 & 1 & 1 & \cdots & 1 \\
            h_1(m-k) & h_1(m-k+1) & h_1(m-k+2) & \cdots & h_1(m-k+r) \\
            h_2(m-k) & h_2(m-k+1) & h_2(m-k+2) & \cdots & h_2(m-k+r) \\
            \vdots & \vdots & \vdots &  & \vdots \\
            h_r(m-k) & h_r(m-k+1) & h_r(m-k+2) & \cdots & h_r(m-k+r)
        \end{pmatrix},
    \]
    where $h_i(x) = x(x-1)(x-2)\cdots(x-i+1)$ is a degree $i$ polynomial.

    This matrix is invertible. To see this, let $\alpha_j = m-k-j$. The above matrix is rewritten as 
    \[
        \begin{pmatrix}
            1 & 1 & 1 & \cdots & 1 \\
            h_1(\alpha_0) & h_1(\alpha_1) & h_1(\alpha_2) & \cdots & h_1(\alpha_r) \\
        h_2(\alpha_0) & h_2(\alpha_1) & h_2(\alpha_2) & \cdots & h_2(\alpha_r) \\
            \vdots & \vdots & \vdots &  & \vdots \\
            h_r(\alpha_0) & h_r(\alpha_1) & h_r(\alpha_2) & \cdots & h_r(\alpha_r)
        \end{pmatrix}.
    \]
    Using the smaller degree monomials in the rows above it, the polynomial $h_i$ in each row can iteratively be made into simply the monomial $x^i$. In particular, the rank of the above matrix is the same as the rank of the Vandermonde matrix, which has full rank.
\end{proof}


\begin{lemma}
    Assuming that $p > 2d+2$, it holds that for $j + k > 2d$ and for all $0 \le i \le d$, we have that $c_{ijk} = 0$.
\end{lemma}

\begin{proof}
    We backwards induct on the value of $j + k$ to show that $c_{ijk} = 0~\forall i \in [0, d]$. The base case is $j + k = 2p-1$. In this case, there are no terms with $j + k = 2p-1$, so $c_{ijk} = 0$ for all $i \in [0, d]$ and $j + k = 2p-1$. \rnote{not sure if this is a convincing base case... the relevant point is that no larger terms can interfere}

    Now, assume that for $s > 2d$ and $j + k > s$, it holds that $c_{ijk} = 0~\forall i \le d$. We will prove that $c_{ijk} = 0$ for $i \in [0, d]$ and $j + k = s$.

    \begin{claim}
        Assume that $c_{ijk} = 0$ for $j + k > s$. Then for $\hat{j} + \hat{k} = s$, it holds that
        \[
            g_{\hat{j}\hat{k}}(x) = \sum_{\substack{0 \le i \le d \\ \hat{k} \le k \le p-1}} c_{i,s-k,k} \cdot \binom{k}{\hat{k}} x^{k-\hat{k}+i}. 
        \]
    \end{claim}

    \begin{proof}
        Consider a term $c_{ijk}x^iy^j(xy+z)^k$ that appears in $f(x,y,xy+z)$. This expands to
        \[
            c_{ijk} \cdot \sum_{0 \le k' \le k} \binom{k}{k'} x^{k-k'+i}y^{j+k-k'}z^{k'}.
        \]
        Note that all the sum of the exponents of $y$ and $z$ in all the resulting terms is $(j+k-k') + k' = j+k = s$. Now, looking at $g_{\hat{j}\hat{k}}(x)$, we see that the coefficients $c_{ijk}$ that appear in its expression are those where $(j \modstar{p}) + k = s$. Since we've assumed that $c_{ijk} = 0$ for $j + k > s$, it holds that the $c_{ijk}$ that appear are precisely those where $j + k = s$. Comparing terms, we obtain the formula in the claim.
    \end{proof}

    % \begin{claim}
    %     Assuming that $c_{ijk} = 0~\forall i \le d, j + k > s$, we have that for $j + k = s$ and $i \in [0, d]$, 
    %     \[
    %         g_{\hat{i}\hat{j}\hat{k}} = 
    %     \]
    % \end{claim}
    
    % \begin{proof}
        
    % \end{proof}

    We now prove the inductive step for $j + k = s$. We split into three cases.
    
    \vspace{0.5em}
    \begin{caseof}
    
    \hspace{-3em}
    \case{$s > p-1 + d$.}{
        We proceed by backwards induction on the value of $k$. For $k > p-1$, there are no such terms, so $c_{i,s-k,k} = 0$. \rnote{again the point is that there's no higher terms that can interfere}

        Now assuming that for $k' > k$ all $c_{i,s-k',k'} = 0$, we have that 
        \begin{align*}
            g_{s-k,k}(x) 
            &= \sum_{\substack{0 \le i \le d \\ k \le k' \le p-1}} c_{i,s-k',k'} \cdot \binom{k'}{k} x^{k'-k+i} \\
            &= \sum_{0 \le i \le d} c_{i, s-k, k} \cdot x^i.
        \end{align*}
        This is a polynomial of degree $d < p$, which implies all the coefficients $c_{i, s-k, k} = 0$. This completes the inductive step.
    }
    \vspace{0.5em}
    \case{$p-1 < s \le p-1 + d$.}{
        Consider the following matrix:
        \[
        \kbordermatrix{
            & g_{d+1,s-d-1} & g_{d+2,s-d-2} & g_{d+3,s-d-3} & \cdots & g_{p-1,s-p+1} \\
            c_{i, s-p+1, p-1} & \binom{p-1}{s-d-1} x^{p-s+d+i} & \binom{p-1}{s-d-2} x^{p-s+d+i+1} & \binom{p-1}{s-d-3} x^{p-s+d+i+2} & \cdots & \binom{p-1}{s-p+1} x^{2p-s+i-2} \\
            c_{i, s-p+2, p-2} & \binom{p-2}{s-d-1} x^{p-s+d+i-1} & \binom{p-2}{s-d-2} x^{p-s+d+i} & \binom{p-2}{s-d-3} x^{p-s+d+i+1} & \cdots & \binom{p-2}{s-p+1} x^{2p-s+i-3} \\
            c_{i, s-p+3, p-3} & \binom{p-3}{s-d-1} x^{p-s+d+i-2} & \binom{p-3}{s-d-2} x^{p-s+d+i-1} & \binom{p-3}{s-d-3} x^{p-s+d+i} & \cdots & \binom{p-3}{s-p+1} x^{2p-s+i-4} \\
            \vdots & \vdots & \vdots & \vdots &  & \vdots \\
            c_{i,d+1,s-d-1} & \binom{s-d-1}{s-d-1} x^i & \binom{s-d-1}{s-d-2} x^{i+1} & \binom{s-d-1}{s-d-3} x^{i+2} & \cdots & \binom{s-d-1}{s-p+1} x^{p-d+i-2} \\
            c_{i,d+2,s-d-2} & 0 & \binom{s-d-2}{s-d-2} x^i & \binom{s-d-2}{s-d-3} x^{i+1} & \cdots & \binom{s-d-2}{s-p+1} x^{p-d+i-3} \\
            c_{i,d+3,s-d-3} x^i & 0 & 0 & \binom{s-d-3}{s-d-3} & \cdots & \binom{s-d-3}{s-p+1} x^{p-d+i-4} \\
            \vdots & \vdots & \vdots & \vdots &  & \vdots \\
            c_{i,p-1,s-p+1} & 0 & 0 & 0 & \cdots & \binom{s-p-1}{s-p-1} x^i
        }
        \]
        The rows correspond to the coefficients $c_{i,s-k,k}$ for $k$ in the range $[s-p+1,p-1]$ as labeled on the left. Each row actually corresponds to $d+1$ coefficients, for $i \in [0, d]$, but for sake of space we condense these into a single row. 
        
        The columns correspond to $g_{d',s-d'}(x)$, i.e. the coefficient of $y^{d'}z^{s-d'}$, for $d' \in [d+1, p-1]$. The way to read off the value of $g_{d',s-d'}(x)$ is by looking at the corresponding column, and summing the product of each entry with the corresponding row coefficient $c_{i,s-k',k'}$, remembering that each row actually corresponds to $d+1$ rows for $i \in [0, d]$. 

        % By Lemma~\ref{lemma:invertible_matrix}, any square submatrix with diagonal lying above the bottom left triangle of $0$'s is invertible.

        Now, to prove that $c_{i,s-k,k} = 0$ for all $i \in [0, d]$ and $k \in [0,p-1]$, we will backwards induct on the value of $i+k$. So assume that for $i' + k' > t$ that $c_{i',s-k',k'} = 0$. This is true for $t = d + (p-1)$, since there do not exist coefficients with larger values of $i' + k'$.

        Consider all the coefficients with $i + k = t$, meaning coefficients $c_{i, s-t+i, t-i}$ where $i \in [0, d]$ and $t-i, s-t+i \in [0, p-1]$. These coefficients correspond to $\le d+1$ consecutive rows of the matrix. Furthermore, since the value of $i$ in these coefficients increases by $1$ as you go down the rows of the matrix, while the exponent of $x$ in any column increases by $1$ (relative to $i$) decreases by $1$, these coefficients all belong (and are the only contributors) to the coefficient of $x^{i'}$ for some $i'$ in the value of $g_{d',s-d'}(x)$. Thus, for any $g_{d', s-d'}(x)$ which has degree $< p$, we obtain a linear constraint on $c_{i, s-t+i, t-i}$ by restricting the column corresponding to $g_{d',s-d'}$ to the rows corresponding to the coefficients (we may also drop the powers of $x$, so that the coefficients of the linear constraint are simply binomial coefficients). 

        Our strategy may therefore be summarized as follows: for each $t \le p-1 + d$, assuming that there are $m$ coefficients of the form $c_{i,s-t+i,t-i}$, we will find $m$ consecutive columns such that the degree of $x$ in the corresponding $g_{d',s-d'}(x)$ is $< p$. These columns will also satisfy that if we restrict the matrix to these columns and to the rows corresponding to the coefficients, the resulting $m \times m$ matrix has diagonal that lies above the lower left triangle of $0$'s. Then, by Lemma~\ref{lemma:invertible_matrix}, we know these $m$ linear constraints are independent, telling us that each $c_{i, s-t+i, t-i} = 0$.

        The columns will be chosen as follows:
        \begin{itemize}
        
        \item 
            For $t \ge p-1$, we are considering the $p-t+d$ coefficients 
            \[
                c_{t-p+1, s-p+1, p-1}, c_{t-p+2, s-p+2, p-2}, \dots, c_{d, s-t+d, t-d}.
            \]
            We pick the first $p-t+d$ columns of the matrix, corresponding to $g_{d+1,s-d-1}, g_{d+2,s-d-2}, \dots, g_{p+2d-t,s+t-p-2d}$. Each of $g_{d',s-d'}(x)$ for $d' \in [d+1, p+2d-t]$ is a polynomial in $x$. Using that for $i'+k' > t$ we have that $c_{i',s-k',k'} = 0$, we see that the maximum degree of $x$ in any of these polynomials is $\le i + k - \min (s-d') = t - (s+t-p-2d) = p+2d-s \le 2d < p$.

        \item 
            For $s-d-1 \le t < p-1$, we are looking at the $d+1$ coefficients 
            \[
                c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}.
            \]
            Consider the $d+1$ columns corresponding to $g_{d+1, s-d-1}, \dots, g_{2d+1, s-2d-1}$. The smallest exponent of $x$ is $\ge 0$, and the largest is $\le i + k - (s-2d-1) \le t - s + 2d - 1 \le 2d-1 < p$.

        \item 
            For $t < s - d - 1$, let $\hat{d} = \min(d, p-1-s+t)$. We consider the $\hat{d} + 1$ coefficients
            \[
                c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{\hat{d},s-t+\hat{d},t-\hat{d}}.
            \]
            Look at the $\hat{d} + 1$ columns corresponding to $g_{s-t,t},\dots,g_{s-t+\hat{d},t-\hat{d}}$. The powers of $x$ range from $\ge 0$ to $\le i+k - (t-\hat{d}) \le \hat{d} < p$. 
            
        \end{itemize}

        

        % We now split the analysis into three cases.

        % \begin{subcaseof}
        
        % \subcase{$t > p-1$}{
        %     In this case, we are considering the $p-t+d$ coefficients  
        %     \[
        %         c_{t-p+1, s-p+1, p-1}, c_{t-p+2, s-p+2, p-2}, \dots, c_{d, s-t+d, t-d}.
        %     \]
        %     These coefficients lie in the first $p-t+d$ rows of the matrix. We will find a set of $p-t+d$ linearly independent constraints on these coefficients, which will imply they are all $0$. To do this, we consider the first $p-t+d$ columns of the matrix, corresponding to $g_{d+1,s-d-1}, g_{d+2,s-d-2}, \dots, g_{p+2d-t,s+t-p-2d}$. Each of $g_{d',s-d'}(x)$ for $d' \in [d+1, p+2d-t]$ is a polynomial in $x$. Using that for $i'+k' > t$ we have that $c_{i',s-k',k'} = 0$, we see that the maximum degree of $x$ in any of these polynomials is $\le i + k - \min (s-d') = t - (s+t-p-2d) = p+2d-s \le 2d < p$. Thus, each of the coefficients of $x^{i'}$ in $g_{d',s-d'}(x)$ must be $0$.

        %     In the column corresponding to $g_{d',s-d'}$, we read off the coefficient of $x^{t-s+d'}$. This is chosen so that the coefficients involved are precisely those where $i+k = t$. This will give us precisely the following linear constraints on our coefficients:
        %     \[ 
        %     \begin{pmatrix}
        %         \binom{p-1}{s-d-1} & \binom{p-1}{s-d-2} & \cdots & \binom{p-1}{s+t-p-2d} \\
        %         \binom{p-2}{s-d-1} & \binom{p-2}{s-d-2} & \cdots & \binom{p-2}{s+t-p-2d} \\
        %         \vdots & \vdots &  & \vdots \\
        %         \binom{t-d}{s-d-1} & \binom{t-d}{s-d-2} & \cdots & \binom{t-d}{s+t-p-2d}
        %     \end{pmatrix}^T
        %     \begin{pmatrix}
        %         c_{t-p+1, s-p+1, p-1} \\ 
        %         c_{t-p+2, s-p+2, p-2} \\
        %         \vdots \\
        %         c_{d, s-t+d, t-d}
        %     \end{pmatrix}
        %     = 
        %     \begin{pmatrix}
        %         0 \\
        %         0 \\
        %         \vdots \\
        %         0
        %     \end{pmatrix}.
        %     \]
        %     Note that the left hand matrix is simply the top left $(p-s+d) \times (p-s+d)$ matrix, which is invertible.
        % }

        % \subcase{$s-d-1 \le t \le p-1$.}{
        %     In this case, we are looking at the coefficients 
        %     \[
        %         c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}.
        %     \]
            
        %     Consider the coefficients of $y^{d+1}z^{s-d-1}, \dots, y^{2d+1}z^{s-2d-1}$. The smallest exponent of $x$ is $\ge 0$, and the largest is $\le i + k - (s-2d-1) \le t - s + 2d - 1 \le 2d-1 < p$, so all coefficients of $x^iy^jz^k$ must be $0$. In particular, look at the coefficients of $x^{t-s+d+1}y^{d+1}z^{s-d-1}, \dots, x^{t-s+2d-1}y^{2d+1}z^{s-2d-1}$. This gives us the system of equations:
        %     \[
        %         \begin{pmatrix}
        %             \binom{t}{s-d-1} & \binom{t-1}{s-d-1} & \cdots & \binom{t-d}{s-d-1} \\
        %             \binom{t}{s-d-2} & \binom{t-1}{s-d-2} & \cdots & \binom{t-d}{s-d-2} \\
        %             \vdots & \vdots &  & \vdots \\
        %             \binom{t}{s-2d-1} & \binom{t-1}{s-2d-1} & \cdots & \binom{t-d}{s-2d-1}
        %         \end{pmatrix}
        %         \begin{pmatrix}
        %             c_{0,s-t,t} \\
        %             c_{1,s-t+1,t-1} \\
        %             \vdots \\ 
        %             c_{d,s-t+d,t-d}
        %         \end{pmatrix}
        %         = 
        %         \begin{pmatrix}
        %             0 \\
        %             0 \\
        %             \vdots \\
        %             0
        %         \end{pmatrix}.
        %     \]
        %     Since the left matrix is invertible, we get that all coefficients $c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}$ are $0$.
        % }

        % \end{subcaseof}
        

        % The largest possible value of $i + k$ is $d + p-1$. We look at the coefficient of $y^{d+1}z^{s-d+1}$. The exponents of $x$ range from $0$ to $(p-1)-(s-d-1)+d = p-s+2d \le 2d < p$, so in fact all the coefficients of $x^i$, $i \in [0, p-s+2d]$ must be $0$. If we look at the coefficient of $x^{p-s+2d}y^{d+1}z^{s-d-1}$, we get the term $\binom{p-1}{s-d-1} c_{d, s-p+1, p-1}$, implying that $c_{d, s-p+1, p-1} = 0$.

    %     Now, assume that for $i+k > t$ we've already shown that $c_{i,s-k,k} = 0$. We split the analysis into three cases:
    %     \begin{subcaseof}
    %     \subcase{$t > p-1$}{
    %         In this subcase, we have the coefficients 
    %         \[
    %             c_{t-p+1, s-p+1, p-1}, c_{t-p+2, s-p+2, p-2}, \dots, c_{d, s-t+d, t-d}.
    %         \]
    %         Consider the coefficients of $y^{d+1}z^{s-d-1}, \dots, y^{p+2d-t}z^{s+t-p-2d}$. The smallest exponent of $x$ is $\ge 0$ and the largest is $i+k - (s+t-p-2d) \le p+2d-s \le 2d < p$, where we used that for $i + k > t$ the coefficients are $0$. Thus the coefficients of all $x^{i}y^{d'}z^{s-d'}$ terms, $d' \in [d+1, p+2d-t]$, are $0$. In particular, if we look at the coefficients of $x^{t-s+d+1}y^{d+1}z^{s-d-1}, \dots, x^{p+2d-s}y^{p+2d-t}z^{s+t-p-2d}$, we get the following system of equations:
    %         \[ 
    %         \begin{pmatrix}
    %             \binom{p-1}{s-d-1} & \binom{p-2}{s-d-1} & \cdots & \binom{t-d}{s-d-1} \\
    %             \binom{p-1}{s-d-2} & \binom{p-2}{s-d-2} & \cdots & \binom{t-d}{s-d-2} \\
    %             \vdots & \vdots &  & \vdots \\
    %             \binom{p-1}{s+t-p-2d} & \binom{p-2}{s+t-p-2d} & \cdots & \binom{t-d}{s+t-p-2d}
    %         \end{pmatrix}
    %         \begin{pmatrix}
    %             c_{t-p+1, s-p+1, p-1} \\ 
    %             c_{t-p+2, s-p+2, p-2} \\
    %             \vdots \\
    %             c_{d, s-t+d, t-d}
    %         \end{pmatrix}
    %         = 
    %         \begin{pmatrix}
    %             0 \\
    %             0 \\
    %             \vdots \\
    %             0
    %         \end{pmatrix}.
    %         \]
    %         The left matrix is invertible, so all coefficients with $i + k = t$, $j + k = s$ must be $0$.
    %     }
    %     \subcase{$s-d-1 \le t \le p-1$}{
    %         In this case, we are looking at the coefficients 
    %         \[
    %             c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}.
    %         \]
    %         Consider the coefficients of $y^{d+1}z^{s-d-1}, \dots, y^{2d+1}z^{s-2d-1}$. The smallest exponent of $x$ is $\ge 0$, and the largest is $\le i + k - (s-2d-1) \le t - s + 2d - 1 \le 2d-1 < p$, so all coefficients of $x^iy^jz^k$ must be $0$. In particular, look at the coefficients of $x^{t-s+d+1}y^{d+1}z^{s-d-1}, \dots, x^{t-s+2d-1}y^{2d+1}z^{s-2d-1}$. This gives us the system of equations:
    %         \[
    %             \begin{pmatrix}
    %                 \binom{t}{s-d-1} & \binom{t-1}{s-d-1} & \cdots & \binom{t-d}{s-d-1} \\
    %                 \binom{t}{s-d-2} & \binom{t-1}{s-d-2} & \cdots & \binom{t-d}{s-d-2} \\
    %                 \vdots & \vdots &  & \vdots \\
    %                 \binom{t}{s-2d-1} & \binom{t-1}{s-2d-1} & \cdots & \binom{t-d}{s-2d-1}
    %             \end{pmatrix}
    %             \begin{pmatrix}
    %                 c_{0,s-t,t} \\
    %                 c_{1,s-t+1,t-1} \\
    %                 \vdots \\ 
    %                 c_{d,s-t+d,t-d}
    %             \end{pmatrix}
    %             = 
    %             \begin{pmatrix}
    %                 0 \\
    %                 0 \\
    %                 \vdots \\
    %                 0
    %             \end{pmatrix}.
    %         \]
    %         Since the left matrix is invertible, we get that all coefficients $c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}$ are $0$.
    %     }
    %     \subcase{$t < s-d-1$}{
    %         In this case, let $\hat{d} = \min(d, p-1-s+t)$. We consider the coefficients
    %         \[
    %             c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{\hat{d},s-t+\hat{d},t-\hat{d}}.
    %         \]
    %         Look at the coefficients of $y^{s-t}z^t,\dots,y^{s-t+\hat{d}}z^{t-\hat{d}}$. The powers of $x$ range from $\ge 0$ to $\le i+k - (t-\hat{d}) \le \hat{d} < p$. So we get the following system of equations from looking at the coefficients of $x^{0}y^{s-t}z^t, \dots, x^{\hat{d}}y^{s-t+\hat{d}}z^{t-\hat{d}}$:
    %         \[
    %             \begin{pmatrix}
    %                 \binom{t}{t} & \binom{t-1}{t} & \cdots & \binom{t-\hat{d}}{t} \\
    %                 \binom{t}{t-1} & \binom{t-1}{t-1} & \cdots & \binom{t-\hat{d}}{t-1} \\
    %                 \vdots & \vdots &  & \vdots \\
    %                 \binom{t}{t-\hat{d}} & \binom{t-1}{t-\hat{d}} & \cdots & \binom{t-\hat{d}}{t-\hat{d}}
    %             \end{pmatrix}
    %             \begin{pmatrix}
    %                 c_{0,s-t,t} \\
    %                 c_{1,s-t+1,t-1} \\
    %                 \vdots \\ 
    %                 c_{\hat{d},s-t+\hat{d},t-\hat{d}}
    %             \end{pmatrix}
    %             = 
    %             \begin{pmatrix}
    %                 0 \\
    %                 0 \\
    %                 \vdots \\
    %                 0
    %             \end{pmatrix}.
    %         \]
    %         The left matrix is lower triangular so it is invertible, and we get that $c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{\hat{d},s-t+\hat{d},t-\hat{d}} = 0$.
    %     }
    %     \end{subcaseof}

    %     \rnote{this is the point:}
    %     All the above can be summarized by requiring that certain submatrices of the following are invertible: (matrices are transposed from the above)
    %     \[
    %         \begin{pmatrix}
    %         \binom{p-1}{s-d-1} & \binom{p-1}{s-d-2} & \binom{p-1}{s-d-3} & \cdots & \binom{p-1}{s-p+1} \\
    %         \binom{p-2}{s-d-1} & \binom{p-2}{s-d-2} & \binom{p-2}{s-d-3} & \cdots & \binom{p-2}{s-p+1} \\
    %         \binom{p-3}{s-d-1} & \binom{p-3}{s-d-2} & \binom{p-3}{s-d-3} & \cdots & \binom{p-3}{s-p+1} \\
    %         \vdots & \vdots & \vdots &  & \vdots \\
    %         \binom{s-d-1}{s-d-1} & \binom{s-d-1}{s-d-2} & \binom{s-d-1}{s-d-3} & \cdots & \binom{s-d-1}{s-p+1} \\
    %         0 & \binom{s-d-2}{s-d-2} & \binom{s-d-2}{s-d-3} & \cdots & \binom{s-d-2}{s-p+1} \\
    %         0 & 0 & \binom{s-d-3}{s-d-3} & \cdots & \binom{s-d-3}{s-p+1} \\
    %         \vdots & \vdots & \vdots &  & \vdots \\
    %         0 & 0 & 0 & \cdots & \binom{s-p-1}{s-p-1}
    %         \end{pmatrix}
    %     \]
    %     The submatrices we need are those starting in the upper left corner of size up to $d+1$, those beginning in the $d'$'th row and leftmost column where $d' \le d$, of size $d$, and those beginning at one of the terms labeled $\binom{k}{k}$, and of size $d$ or until they get cut off at the lower right corner. The reason that $s > 2d+2$ is important is because this ensures that there are at least $(s-d-1)-(s-p+1) + 1 = p-d-1 > d+1$ columns and thus $\ge d+1$ linearly independent equations.
    }
    \vspace{0.5em}
    \case{$2d < s \le p-1$}{
        Similar to the previous case, we consider the following matrix:
        \begin{align*}
            \kbordermatrix{
            & g_{d+1,s-d-1} & g_{d+2,s-d-2} & g_{d+3,s-d-3} & \cdots & g_{s,0} \\
            c_{i,0,s} & \binom{s}{s-d-1} x^{i+d+1} & \binom{s}{s-d-2} x^{i+d+2} & \binom{s}{s-d-3} x^{i+d+3} & \cdots & \binom{s}{0} x^{i+s} \\
            c_{i,1,s-1} & \binom{s-1}{s-d-1} x^{i+d} & \binom{s-1}{s-d-2} x^{i+d+1} & \binom{s}{s-d-3} x^{i+d+2} & \cdots & \binom{s-1}{0} x^{i+s-1} \\
            c_{i,2,s-2} & \binom{s-2}{s-d-1} x^{i+d-1} & \binom{s-2}{s-d-2} x^{i+d} & \binom{s-2}{s-d-3} x^{i+d-1} & \cdots & \binom{s-2}{0} x^{i+s-2} \\
            \vdots & \vdots & \vdots &  & \vdots \\
            c_{i,d+1,s-d-1} & \binom{s-d-1}{s-d-1} x^{i} & \binom{s-d-1}{s-d-2} x^{i+1} & \binom{s-d-1}{s-d-3} x^{i+2} & \cdots & \binom{s-d-1}{0} x^{i+s-d-1} \\
            c_{i,d+2,s-d-2} & 0 & \binom{s-d-2}{s-d-2} x^i & \binom{s-d-2}{s-d-3} x^{i+1} & \cdots & \binom{s-d-2}{0} x^{i+s-d-2} \\
            c_{i,d+3,s-d-3} & 0 & 0 & \binom{s-d-3}{s-d-3} x^i & \cdots & \binom{s-d-3}{0} x^{i+s-d-3} \\
            \vdots & \vdots & \vdots &  & \vdots \\
            c_{i,s,0} & 0 & 0 & 0 & \cdots & \binom{0}{0} x^i
            }.
        \end{align*}
        As in the previous case, we will downwards induct on the value of $i + k = t$. Assume that for $i' + k' > t$ it holds that $c_{i',s-k',k'} = 0$. This is true for $t = d + s$ (the maximal possible value of $i+k$) since there do not exist coefficients with larger values of $i' + k'$.

        We again consider all $m$ coefficients satisfying $i + k = t$. These occupy a number of consecutive rows of the matrix. Furthermore, for any column with degree in $x$ less than $p$, restricting that column to those rows gives a linear constraint on the coefficients. Thus, we again demonstrate, for each $t$, $m$ consecutive columns that each have exponent in $x$ less than $p$. Restricting these columns to the coefficient rows will result in a $m \times m$ submatrix lying above the lower left triangle of $0$'s, which is full rank by Lemma~\ref{lemma:invertible_matrix}, implying that all $m$ coefficients must in fact be $0$.

        \begin{itemize}
        \item 
            For $t \ge s$, we consider the $s-t+d+1$ coefficients 
            \[
                c_{t-s,0,s}, c_{t-s+1,1,s-1}, \dots, c_{d,s-t+d,t-d}.
            \]
            Look at the first $s-t+d+1$ columns corresponding to $g_{d', s-d'}$ for $d' \in [d+1, s-t+2d+1]$. The maximum degree of any of these polynomials is $i + k - (t-2d-1) \le 2d+1 < p$.

        \item 
            For $s-d-1 \le t < s$, we consider the $d+1$ coefficients
            \[
                c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{d,s-t+d,t-d}.
            \]
            Look at the $d+1$ columns $g_{d+1,s-d-1}, \dots, g_{2d+1,s-2d-1}$. The maximum degree of any of these polynomials is $\le i + k - (s-2d-1) = t - s + 2d + 1 < 2d+1 < p$.

        \item 
            For $t < s-d-1$, let $\hat{d} = \min(d, t)$. Then we are considering the following $\hat{d} + 1$ coefficients.
            \[
                c_{0,s-t,t}, c_{1,s-t+1,t-1}, \dots, c_{\hat{d}, s-t+\hat{d}, t-\hat{d}}.
            \]
            For these, we will look at the $\hat{d}+1$ columns corresponding to $g_{s-t,t}, \dots, g_{s-t+\hat{d},t-\hat{d}}$. The maximum degree of $x$ in any of these polynomials is $i + k - (t-\hat{d}) = \hat{d} < p$.
        \end{itemize}
        
        % The submatrices we need are those starting in the upper left corner of size up to $d+1$, those beginning in the $d'$'th row and leftmost column where $d' \le d$, of size $d$, and those beginning at one of the terms labeled $\binom{k}{k}$, and of size $d$ or until they get cut off at the lower right corner. The reason that $s > 2d+2$ is important is because this ensures that there are at least $d+1$ columns, and thus $d+1$ linearly independent equations, to rule out each tuple of up to $d+1$ coefficients.
    }
    \end{caseof}
    
    % We will show by induction again that $c_{ijk} = 0~\forall i$, this time inducting from $k = p$. Clearly for $k = p$ we have that $c_{ijk} = 0$. Now assume that for all $k' \ge k$ and $j' = p-1+s - k'$ it holds that $c_{i'j'k'} = 0$ for all $0 \le i' \le d$. 
    % \begin{align*}
    %     g_{s, p-1}(x) &= \sum_{0 \le i \le d} c_{i,s,p-1} \cdot x^i \\
    %     g_{s+1, p-2}(x) &= \sum_{0 \le i \le d} c_{i, s+1, p-2} \cdot x^i + \sum_{0 \le i \le d} c_{i,s,p-1} \cdot (p-1) x^{i+1}
    % \end{align*}
\end{proof}

\begin{lemma} \label{lemma:rate}
    The dimension of the code is $(d+1)^3$.
\end{lemma}

\begin{proof}
    
\end{proof}



==> unused/macros.tex <==
% {{{ etex }}}

\usepackage{etex}

% {{{ nag }}}

\usepackage[l2tabu, orthodox]{nag}


% {{{ common }}}

\usepackage{xspace,enumerate}

\usepackage[dvipsnames]{xcolor}

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}

% {{{ babelamerican }}}

\usepackage[american]{babel}


% {{{ mathtools }}}

\usepackage{mathtools}


% {{{ boldmath }}}

% fix for "too many math alphabets" problem
\newcommand\hmmax{0} % default 3
%\usepackage{bm}

\usepackage{stmaryrd}


% {{{ amsthm }}}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{itheorem}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{fact*}{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{reduction}[theorem]{Reduction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}

% {{{ repeating a theorem }}}

\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 ##1}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}
}



% {{{ geometry-nice }}}


% nicer margins  (lines are not as long)
\usepackage[letterpaper,
top=1.3in,
bottom=1.3in,
left=1.6in,
right=1.6in]{geometry}

% smaller margin for submission?
% \usepackage[letterpaper,
% top=1in,
% bottom=1in,
% left=1in,
% right=1in]{geometry}


% {{{ pxfonts }}}

\usepackage[varg]{pxfonts} % varg - uses nicer g,v,y,w

%\usepackage[sc,osf]{mathpazo}
\usepackage{tgpagella}
\usepackage{lmodern}

% {{{ showkeys }}}

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi

% {{{ hyperref-option2 }}}

\ifnum\showcolorlinks=1
\usepackage[
pagebackref,
letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
]{hyperref}
\fi

\ifnum\showcolorlinks=0
\usepackage[
pagebackref,
letterpaper=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}
\fi


% {{{ prettyref }}}
\usepackage{prettyref}

% From manual:
% \newrefformat{eq}{\textup{(\ref{#1})}}
% \newrefformat{lem}{Lemma~\ref{#1}}
% \newrefformat{thm}{Theorem~\ref{#1}}
% \newrefformat{cha}{Chapter~\ref{#1}}
% \newrefformat{sec}{Section~\ref{#1}}
% \newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
% \newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}

\newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}

\newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
\newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
\newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
\newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
\newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
\newrefformat{cha}{\savehyperref{#1}{Chapter~\ref*{#1}}}
\newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
\newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
\newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
\newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
\newrefformat{hyp}{\savehyperref{#1}{Hypothesis~\ref*{#1}}}
\newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
\newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
\newrefformat{item}{\savehyperref{#1}{Item~\ref*{#1}}}
\newrefformat{step}{\savehyperref{#1}{step~\ref*{#1}}}
\newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
\newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
\newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
\newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
\newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
\newrefformat{relax}{\savehyperref{#1}{Relaxation~\ref*{#1}}}
\newrefformat{red}{\savehyperref{#1}{Reduction~\ref*{#1}}}
\newrefformat{part}{\savehyperref{#1}{Part~\ref*{#1}}}



% {{{ sref }}}

% short section reference
\newcommand{\Sref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% {{{ nicefrac }}}
% commands for fractions
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}




% {{{ microtype-option }}}

\ifnum\usemicrotype=1
\usepackage{microtype}
\fi


% {{{ authornotes }}}
\ifnum\showauthornotes=1
\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\Authornotecolored}[3]{{\small\color{#1}{[#2: #3]}}}
\newcommand{\Authorcomment}[2]{{\sffamily\small\color{gray}{[#1: #2]}}}
\newcommand{\Authorstartcomment}[1]{\sffamily\small\color{gray}[#1: }
\newcommand{\Authorendcomment}{]\rmfamily\normalsize\color{black}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\newcommand{\Authorfixme}[1]{\Authornote{#1}{\textbf{??}}}
\newcommand{\Authormarginmark}[1]{\marginpar{\textcolor{red}{\fbox{\Large #1:!}}}}
\else
\newcommand{\Authornote}[2]{}
\newcommand{\Authornotecolored}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorstartcomment}[1]{}
\newcommand{\Authorendcomment}{}
\newcommand{\Authorfnote}[2]{}
\newcommand{\Authorfixme}[1]{}
\newcommand{\Authormarginmark}[1]{}
\fi

\newcommand{\Dnote}{\Authornote{D}}
\newcommand{\Inote}{\Authornotecolored{blue}{Irit}}
\newcommand{\inote}{\Inote}
\newcommand{\Gnote}{\Authornote{G}}
\newcommand{\Icomment}{\Authorcomment{I}}
\newcommand{\Dcomment}{\Authorcomment{D}}
\newcommand{\Dstartcomment}{\Authorstartcomment{D}}
\newcommand{\Dendcomment}{\Authorendcomment}
\newcommand{\Dfixme}{\Authorfixme{D}}
\newcommand{\Dmarginmark}{\Authormarginmark{D}}
\newcommand{\Dfnote}{\Authorfnote{D}}

\newcommand{\Pnote}{\Authornote{P}}
\newcommand{\Pfnote}{\Authorfnote{P}}

\newcommand{\PRnote}{\Authornote{PR}}
\newcommand{\PRfnote}{\Authorfnote{PR}}

\newcommand{\PTnote}{\Authornote{PT}}
\newcommand{\PTfnote}{\Authorfnote{PT}}

\newcommand{\PGnote}{\Authornote{PG}}
\newcommand{\PGfnote}{\Authorfnote{PG}}

\newcommand{\Bnote}{\Authornote{B}}
\newcommand{\Bfnote}{\Authorfnote{B}}

\newcommand{\Mnote}{\Authornote{M}}
\newcommand{\Mfnote}{\Authorfnote{M}}

\newcommand{\Rnote}{\Authornote{M}}
\newcommand{\Rfnote}{\Authorfnote{M}}

\newcommand{\Nnote}{\Authornote{N}}
\newcommand{\Nfnote}{\Authorfnote{N}}

\newcommand{\onote}{\Authornote{O}}
\newcommand{\Onote}{\Authornote{O}}

\newcommand{\Snote}{\Authornote{S}}
\newcommand{\Sfnote}{\Authorfnote{S}}


% {{{ fixme }}}

% place red exclamation mark in margin
%\newcommand{\redmarginmarker}{\marginpar{\textcolor{red}{\fbox{\Large !}}}}
\newcommand{\redmarginmarker}{}

% short indicator for places that need fixing
\newcommand{\FIXME}{\textbf{\textcolor{red}{??}}\redmarginmarker}

\ifnum\showfixme=0
\renewcommand{\FIXME}{}
\fi


% {{{ boxedminipage }}}
\usepackage{boxedminipage}

\newenvironment{mybox}
{\center \noindent\begin{boxedminipage}{1.0\linewidth}}
{\end{boxedminipage}
\noindent
}


% {{{ parentheses }}}
% various bracket-like commands
% round parentheses
\newcommand{\paren}[1]{(#1)}
\newcommand{\Paren}[1]{\left(#1\right)}
\newcommand{\bigparen}[1]{\big(#1\big)}
\newcommand{\Bigparen}[1]{\Big(#1\Big)}
% square brackets
\newcommand{\brac}[1]{[#1]}
\newcommand{\Brac}[1]{\left[#1\right]}
\newcommand{\bigbrac}[1]{\big[#1\big]}
\newcommand{\Bigbrac}[1]{\Big[#1\Big]}
% absolute value
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigabs}[1]{\Big\lvert#1\Big\rvert}
% cardinality
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigcard}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigcard}[1]{\Big\lvert#1\Big\rvert}
% set
\newcommand\sett[2]{\left\{ #1 \left| \; \vphantom{#1 #2} \right. #2  \right\}}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\big\{#1\big\}}
\newcommand{\Bigset}[1]{\Big\{#1\Big\}}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\big\lVert#1\big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert#1\Big\rVert}
% 2-norm
\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\Normt}[1]{\Norm{#1}_2}
\newcommand{\bignormt}[1]{\bignorm{#1}_2}
\newcommand{\Bignormt}[1]{\Bignorm{#1}_2}
% 2-norm squared
\newcommand{\snormt}[1]{\norm{#1}^2_2}
\newcommand{\Snormt}[1]{\Norm{#1}^2_2}
\newcommand{\bigsnormt}[1]{\bignorm{#1}^2_2}
\newcommand{\Bigsnormt}[1]{\Bignorm{#1}^2_2}
% norm squared
\newcommand{\snorm}[1]{\norm{#1}^2}
\newcommand{\Snorm}[1]{\Norm{#1}^2}
\newcommand{\bigsnorm}[1]{\bignorm{#1}^2}
\newcommand{\Bigsnorm}[1]{\Bignorm{#1}^2}
% 1-norm
\newcommand{\normo}[1]{\norm{#1}_1}
\newcommand{\Normo}[1]{\Norm{#1}_1}
\newcommand{\bignormo}[1]{\bignorm{#1}_1}
\newcommand{\Bignormo}[1]{\Bignorm{#1}_1}
% infty-norm
\newcommand{\normi}[1]{\norm{#1}_\infty}
\newcommand{\Normi}[1]{\Norm{#1}_\infty}
\newcommand{\bignormi}[1]{\bignorm{#1}_\infty}
\newcommand{\Bignormi}[1]{\Bignorm{#1}_\infty}
% inner product
\newcommand{\iprod}[1]{\langle#1\rangle}
\newcommand{\Iprod}[1]{\left\langle#1\right\rangle}
\newcommand{\bigiprod}[1]{\big\langle#1\big\rangle}
\newcommand{\Bigiprod}[1]{\Big\langle#1\Big\rangle}
% dim
\def\dim{{\rm dim}}
\def\sp{{\rm span}}

% {{{ probability }}}
% expectation, probability, variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}
\newcommand{\Plusymb}{\mathbb{P}\mathrm{lurality}}

\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}
\DeclareMathOperator*{\PluOp}{\Plusymb}
\renewcommand{\Pr}{\ProbOp}
\def\one{{\mathbf{1}}}

% TODO: make case distinction if optional argument is not set
\newcommand{\prob}[1]{\Pr\set{#1}}
\newcommand{\Prob}[2][]{\Pr_{{#1}}\left[#2\right]} % use by \Prob[x]{event}

\newcommand{\ex}[1]{\E\brac{#1}}
\newcommand{\Ex}[2][]{\E_{{#1}}\Brac{#2}}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}

\newcommand{\plu}[2]{\PluOp_{{#1}}{[{#2}}]}
\newcommand{\given}{\;\middle\vert\;}
\newcommand{\ve}{\;\hbox{and}\;}

% {{{ mathfonts }}}

 \usepackage{dsfont}
%\usepackage{yfonts}
\usepackage{mathrsfs}


% {{{ miscmacros }}}

% middle delimiter in the definition of a set
\newcommand{\suchthat}{\;\vert\;}

% tensor product
\newcommand{\tensor}{\otimes}

% add explanations to math displays
\newcommand{\where}{\text{where}}
\newcommand{\textparen}[1]{\text{(#1)}}
\newcommand{\using}[1]{\textparen{using #1}}
\newcommand{\smallusing}[1]{\text{(\small using #1)}}
\ifx\because\undefined
\newcommand{\because}[1]{\textparen{because #1}}
\else
\renewcommand{\because}[1]{\textparen{because #1}}
\fi
\newcommand{\by}[1]{\textparen{by #1}}


% spectral order (Loewner order)
\newcommand{\sge}{\succeq}
\newcommand{\sle}{\preceq}

% smallest and largest eigenvalue
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}

\newcommand{\signs}{\set{1,-1}}
\newcommand{\varsigns}{\set{\pm 1}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\subjectto}{\mathop{\textrm{subject to}}}

\renewcommand{\ij}{{ij}}

% symmetric difference
\newcommand{\symdiff}{\Delta}
\newcommand{\varsymdiff}{\bigtriangleup}

% set of bits
\newcommand{\bits}{\mathbb{F}_2}
\newcommand{\sbits}{\{\pm1\}}

% no stupid bullets for itemize environmentx
\renewcommand{\labelitemi}{--}

% control white space of list and display environments
\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

% short for emptyset
%\newcommand{\eset}{\emptyset}
% moved to mathabbreviations

% short for epsilon
%\newcommand{\e}{\epsilon}
% moved to mathabbreviations

% super index with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% tensor power notation
\newcommand{\tensorpower}[2]{#1^{\tensor #2}}


% multiplicative inverse
\newcommand{\inv}[1]{{#1^{-1}}}

% dual element
\newcommand{\dual}[1]{{#1^*}}

% subset
%\newcommand{\sse}{\subseteq}
% moved to mathabbreviations

% vertical space in math formula
\newcommand{\vbig}{\vphantom{\bigoplus}}

% setminus
\newcommand{\sm}{\setminus}

% define something by an equation (display)
\newcommand{\defeq}{\stackrel{\mathrm{def}}=}
\newcommand{\eqdef}{\stackrel{\mathrm{\Delta}}=}

% define something by an equation (inline)
\newcommand{\seteq}{\mathrel{\mathop:}=}

% declare function f by $f \from X \to Y$
\newcommand{\from}{\colon}

% big middle separator (for conditioning probability spaces)
\newcommand{\bigmid}{~\big|~}
\newcommand{\Bigmid}{~\Big|~}
\newcommand{\Mid}{\;\middle\vert\;}

% better vector definition and some variations
\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\bvec}[1]{\bar{\vec{#1}}}
\newcommand{\pvec}[1]{\vec{#1}'}
\newcommand{\tvec}[1]{{\tilde{\vec{#1}}}}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

% inner product for matrices
\newcommand\bdot\bullet

% transpose
\newcommand{\trsp}[1]{{#1}^\dagger}

% indicator function / vector
%\ifx\mathds\undefined % use double stroke fonts if available
\newcommand{\Ind}{\mathbb I}
%\else
%\newcommand{\Ind}{\mathds 1}
%\fi

% place a qed symbol inside display formula
%\qedhere

% {{{ superscripts }}}

\renewcommand{\th}{\textsuperscript{th}\xspace}
\newcommand{\st}{\textsuperscript{st}\xspace}
\newcommand{\nd}{\textsuperscript{nd}\xspace}
\newcommand{\rd}{\textsuperscript{rd}\xspace}


% {{{ mathoperators }}}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\sdp}{sdp}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\qpoly}{qpoly}
\DeclareMathOperator{\qpolylog}{qpolylog}
\DeclareMathOperator{\qqpoly}{qqpoly}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Conv}{Conv}

\DeclareMathOperator{\rank}{rank}

% operators with limits
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\Median}{Median}

% smaller summation/product symbols
\DeclareMathOperator*{\varsum}{{\textstyle \sum}}
\DeclareMathOperator{\tsum}{{\textstyle \sum}}

\let\varprod\undefined

\DeclareMathOperator*{\varprod}{{\textstyle \prod}}
\DeclareMathOperator{\tprod}{{\textstyle \prod}}




% {{{ differentials }}}

\newcommand{\diffmacro}[1]{\,\mathrm{d}#1}

\newcommand{\dmu}{\diffmacro{\mu}}
\newcommand{\dgamma}{\diffmacro{\gamma}}
\newcommand{\dlambda}{\diffmacro{\lambda}}
\newcommand{\dx}{\diffmacro{x}}
\newcommand{\dt}{\diffmacro{t}}



% {{{ textabbreviations }}}

% some abbreviations
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\phd}{Ph.\,D.\xspace}
\newcommand{\msc}{M.\,S.\xspace}
\newcommand{\bsc}{B.\,S.\xspace}

\newcommand{\etal}{et al.\xspace}

\newcommand{\iid}{i.i.d.\xspace}

% {{{ foreignwords }}}

\newcommand\naive{na\"{\i}ve\xspace}
\newcommand\Naive{Na\"{\i}ve\xspace}
\newcommand\naively{na\"{\i}vely\xspace}
\newcommand\Naively{Na\"{\i}vely\xspace}



% {{{ names }}}
% Hungarian/Polish/East European names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Hastad}{H{\aa}stad\xspace}
\newcommand{\Hoelder}{H\"{o}lder}

% {{{ numbersets }}}
% number sets
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\Rnn}{\R_+}
\newcommand{\varR}{\Re}
\newcommand{\varRnn}{\varR_+}
\newcommand{\varvarRnn}{\R_{\ge 0}}


% {{{ problems }}}

% macros to denote computational problems

% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\texorpdfstring{\textsc{#1}}{#1}\xspace}

% list of problems
\newcommand{\uniquegames}{\problemmacro{unique games}}
\newcommand{\maxcut}{\problemmacro{max cut}}
\newcommand{\multicut}{\problemmacro{multi cut}}
\newcommand{\vertexcover}{\problemmacro{vertex cover}}
\newcommand{\balancedseparator}{\problemmacro{balanced separator}}
\newcommand{\maxtwosat}{\problemmacro{max $2$-sat}}
\newcommand{\maxthreesat}{\problemmacro{max $3$-sat}}
\newcommand{\maxthreelin}{\problemmacro{max $3$-lin}}
\newcommand{\threesat}{\problemmacro{$3$-sat}}
\newcommand{\labelcover}{\problemmacro{label cover}}
\newcommand{\setcover}{\problemmacro{set cover}}
\newcommand{\maxksat}{\problemmacro{max $k$-sat}}
\newcommand{\mas}{\problemmacro{maximum acyclic subgraph}}
\newcommand{\kwaycut}{\problemmacro{$k$-way cut}}
\newcommand{\sparsestcut}{\problemmacro{sparsest cut}}
\newcommand{\betweenness}{\problemmacro{betweenness}}
\newcommand{\uniformsparsestcut}{\problemmacro{uniform sparsest cut}}
\newcommand{\grothendieckproblem}{\problemmacro{Grothendieck problem}}
\newcommand{\maxfoursat}{\problemmacro{max $4$-sat}}
\newcommand{\maxkcsp}{\problemmacro{max $k$-csp}}
\newcommand{\maxdicut}{\problemmacro{max dicut}}
\newcommand{\maxcutgain}{\problemmacro{max cut gain}}
\newcommand{\smallsetexpansion}{\problemmacro{small-set expansion}}
\newcommand{\minbisection}{\problemmacro{min bisection}}
\newcommand{\minimumlineararrangement}{\problemmacro{minimum linear arrangement}}
\newcommand{\maxtwolin}{\problemmacro{max $2$-lin}}
\newcommand{\gammamaxlin}{\problemmacro{$\Gamma$-max $2$-lin}}
\newcommand{\basicsdp}{\problemmacro{basic sdp}}
\newcommand{\dgames}{\problemmacro{$d$-to-$1$ games}}
\newcommand{\maxclique}{\problemmacro{max clique}}
\newcommand{\densestksubgraph}{\problemmacro{densest $k$-subgraph}}


% {{{ alphabet }}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}

\newcommand{\sfE}{\mathsf E}


% {{{ leqslant }}}
% slanted lower/greater equal signs
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}


% {{{ draftbox }}}
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
%        \begin{Large}%
          \Large\textsc{Working Draft}\\%
%        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi


% {{{ varepsilon }}}

\let\epsilon=\varepsilon

% {{{ numberequationwithinsection }}}
\numberwithin{equation}{section}


% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \newcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


% {{{ bibliography }}}

% add section for references to table of contents
\newcommand{\addreferencesection}{
  \phantomsection
  \addcontentsline{toc}{section}{References}
}


% {{{ mathabbreviations }}}

\newcommand{\la}{\leftarrow}
\newcommand{\sse}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\eset}{\emptyset}


% {{{ paragraphperiod }}}


\let\origparagraph\paragraph
\renewcommand{\paragraph}[1]{\origparagraph{#1.}}


% {{{ allowdisplaybreaks }}}
% allows page breaks in large display math formulas

\allowdisplaybreaks



% {{{ sloppy }}}
% avoid math spilling on margin

\sloppy



% {{{ complexityclasses }}}

\newcommand{\cclassmacro}[1]{\texorpdfstring{\textbf{#1}}{#1}\xspace}
\newcommand{\p}{\cclassmacro{P}}
\newcommand{\np}{\cclassmacro{NP}}
\newcommand{\subexp}{\cclassmacro{SUBEXP}}

